Monitoring crop phenology with street-level imagery using computer vision

Street-level imagery holds a significant potential to scale-up in-situ data collection. This is enabled by combining the use of cheap high quality cameras with recent advances in deep learning compute solutions to derive relevant thematic information. We present a framework to collect and extract crop type and phenological information from street level imagery using computer vision. During the 2018 growing season, high definition pictures were captured with side-looking action cameras in the Flevoland province of the Netherlands. Each month from March to October, a fixed 200-km route was surveyed collecting one picture per second resulting in a total of 400,000 geo-tagged pictures. At 220 specific parcel locations detailed on the spot crop phenology observations were recorded for 17 crop types. Furthermore, the time span included specific pre-emergence parcel stages, such as differently cultivated bare soil for spring and summer crops as well as post-harvest cultivation practices, e.g. green manuring and catch crops. Classification was done using TensorFlow with a well-known image recognition model, based on transfer learning with convolutional neural networks (MobileNet). A hypertuning methodology was developed to obtain the best performing model among 160 models. This best model was applied on an independent inference set discriminating crop type with a Macro F1 score of 88.1% and main phenological stage at 86.9% at the parcel level. Potential and caveats of the approach along with practical considerations for implementation and improvement are discussed. The proposed framework speeds up high quality in-situ data collection and suggests avenues for massive data collection via automated classification using computer vision.

==> oldText.tex <==





%\label{S:1}
%\subsection{In-situ data need}
%

%



% Deep learning in agriculture

%\citet{kamilaris2018deep} reviewed studies using deep learning in agriculture and analyzed 40 papers published between 2015 and 2017. The most popular areas are (i) identification of weeds, (ii) land cover classification, (iii) plant recognition, (iv) fruits counting and (vi) crop type classification. Most of the studies focusing on crop identification and crop phenology are using satellite remote sensing (e.g. REF).

%\citet{liakos2018machine}
% Image Data Base 

%\subsection{Plant Recognition with Deep Learning}
% Not specific to agriculture



% Plantnet
% Specific to agriculture
%Specifically in the agriculture domain, the interest to have efficient and effective computer vision algorithms, able of classifying, detecting, or segmenting objects of relevance is huge. Financially agriculture is multi-billion dollar industry (); environmentally it has been linked to major detrimental effects on nature(); and technologically there is an over-reaching impetus to modernize and automate the process like never before. The push for modernization in particular is going very much in the direction of robot-harvesters, equipped with all the sensors needed to locate, extract and store the relevant crop. 
%To name a few examples - we have attempts to automatically identify maize cultivars \citet{lu2016toward}, to classify types of legumes (beans) from leaf vein images \citet{larese2014automatic}, and to recognize greenhouse cucumber fruits \citet{zhang2007recognition}. Indeed, studies exist, where the level of detail is further magnified from mere plant recognition in terms of species, to the next taxonomic grain - variety (\citet{champ2016categorizing}). It should not come as a surprise that in the coming years and decades, there will be plenty more research in this area.

%\citet{waldchen2018automated}


% LeafNet
%\citet{barre2017leafnet}

%\subsection{Phenology Recognition with Deep Learning}
%It seems like a next step in the evolution of these applications would be to go deeper further into the detail tree. In this sense 
%Creating an architecture that can automatically identify not just the species or the variety of the plant, but also its current phenological stage would be an adequate step towards a new state-of-the-art. Phenology is the study of the (inter-) annual life cycle of natural phenomena. When talking about plant phenology we are interested in the recurring stages of development of plants. It is obvious that this study necessarily requires a temporal element and a high enough density of images during the growing season taken at different dates. Steps in this direction have definitely been taken, whereby \citet{yalcin2015phenology} demonstrated the ability to use Histogram Orientated Gradients (HOG) and Gray Level Co-occurance Matrix (GLCM) to recognize and classify phenological stages of several plant species. Although certainly methods from the computer vision domain, HOG and GLCM are texture analysis tools and as such are not the product of a learning algorithm, as much as they are feature extractors from varying neighbourhoods of pixel values. The authors' following work went the \ac{CNN} route and in \citet{yalcin2017plant} were able to achieve good accuracy results for five different crop types in Turkey.
%To the best of our knowledge a labelled open free-of-charge dataset for tracking phenology, so we are extremely happy to share ours. 
%\citet{namin2017deep,namin2018deep}





% % latex table generated in R 3.4.3 by xtable 1.8-2 package
% % Wed Sep 25 16:02:31 2019
% \begin{table}[ht]
% \centering
% \begin{tabular}{rlll}
%   \hline
%  & Old class & Description & New class \\ 
%   \hline
% 1 & BSO1 & class added by surveyors & BSO0 \\ 
%   2 & BSO2 & class added by surveyors & BSO0 \\ 
%   3 & BSO3 & class added by surveyors & BSO0 \\ 
%   4 & BSO4 & class added by surveyors & BSO0 \\ 
%   5 & BSO5 & class added by surveyors & BSO0 \\ 
%   6 & BSO6 & class added by surveyors & BSO0 \\ 
%   7 & ONI0 & pre-emergence class & BSO0 \\ 
%   8 & POT0 & pre-emergence class & BSO0 \\ 
%   9 & SBT0 & pre-emergence class & BSO0 \\ 
%   10 & WWH0 & pre-emergence class & BSO0 \\ 
%   11 & GRA2 & class added by surveyors & GRA1 \\ 
%   12 & GRA3 & class added by surveyors & GRA1 \\ 
%   13 & ONI41 & leaf basis thicken and expand & ONI4 \\ 
%   14 & ONI45 & 50\% of expected bulb/shaft diameter reached & ONI48 \\ 
%   15 & SBT11 & first pair of leaves visible; not yet unfolded & SBT1 \\ 
%   16 & WWH8 & ripening & WWH9 \\ 
%   \hline
% \end{tabular}
% \caption{Class generalizations}
% \label{tab:generalizations}
% \end{table}

% % latex table generated in R 3.4.3 by xtable 1.8-2 package
% % Wed Apr  3 13:57:27 2019
% \begin{table}[ht]
% \centering
% \caption{Number of field observations per date and by crop}
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{rrrrrrrrrrrrrrrrrr}
%   \hline
%  & BSO & CAR & GMA & GRA & GRS & MAI & ONI & POT & SBA & SBT & SCR & SWH & TLP & VEG & WBA & WCR & WWH \\ 
%   \hline
% 2018-03-23 & 150 &   0 &   0 &  26 &   0 &   0 &   4 &   0 &   0 &   1 &  11 &   0 &  10 &   0 &   0 &   0 &  16 \\ 
%   2018-04-23 &  78 &  10 &   0 &  23 &   0 &   1 &  20 &  18 &   0 &  26 &  22 &   0 &  10 &   0 &   0 &   0 &  19 \\ 
%   2018-05-21 &  33 &  12 &   0 &  28 &   0 &  21 &  23 &  43 &   0 &  31 &  17 &   0 &   6 &   0 &   0 &   0 &  18 \\ 
%   2018-06-20 &   6 &  30 &   0 &  27 &   0 &  25 &  24 &  28 &   6 &  30 &   0 &   8 &   4 &   4 &   1 &   0 &  19 \\ 
%   2018-07-09 &   8 &  31 &   0 &  28 &   1 &  25 &  26 &  27 &   7 &  30 &   0 &   8 &   0 &   9 &   0 &   0 &  19 \\ 
%   2018-08-15 &  49 &  30 &   0 &  28 &   0 &  24 &  22 &  26 &   1 &  31 &   0 &   0 &   0 &   8 &   0 &   0 &   0 \\ 
%   2018-09-20 & 111 &  26 &   0 &  29 &   0 &   4 &   0 &  11 &   0 &  30 &   0 &   0 &   0 &   8 &   0 &   0 &   0 \\ 
%   2018-10-17 &  59 &  26 &  44 &  51 &   0 &   0 &   0 &   1 &   0 &  17 &   0 &   0 &   6 &   9 &   0 &   6 &   0 \\ 
%   \hline
% \end{tabular}
% }
% \label{tab:numFOdataNcrop}
% \end{table}

%Table \ref{tab:numFOdataNcrop} shows how many field observations were done in total per crop for the separate field campaigns. We can see that in the beginning and the end of the season the most predominantly surveyed field is of type bare soil, which is understandable as the crops have not yet begun to grow and are not distinguishable. As the season progresses a more nuanced picture appears, whereby the crops in season begin to have a near equal number of observations. 

% \begin{table}[!h]
% \centering
% \footnotesize
% \caption{Number of field observations per crop and by BBCH stage}
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{rrrrrrrrrrrrrrrrrrrrrr}
%   \hline
%  & 0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 11 & 12 & 14 & 19 & 29 & 32 & 39 & 41 & 45 & 48 & 49 \\ 
%   \hline
% Bare Soil & 37 & 24 & 24 & 107 & 45 & 24 & 63 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\ 
%   Carrot & 8 & 73 & 2 & 1 & 29 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\ 
%   Grassland & 1 & 17 & 115 & 27 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\ 
%   Maize & 2 & 20 & 0 & 43 & 0 & 4 & 3 & 23 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\ 
%   Onions & 20 & 46 & 0 & 0 & 2 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 17 & 8 & 21 & 5 \\ 
%   Potatoes & 30 & 28 & 4 & 12 & 0 & 1 & 24 & 0 & 30 & 13 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\ 
%   Sugar beet & 16 & 11 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 2 & 0 & 27 & 1 & 0 & 1 & 91 & 0 & 0 & 0 & 0 \\ 
%   Summer barley & 0 & 0 & 0 & 1 & 0 & 5 & 0 & 1 & 3 & 4 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\ 
%   Summer cereals & 0 & 12 & 22 & 16 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\ 
%   Summer wheat & 0 & 0 & 0 & 0 & 0 & 8 & 0 & 6 & 1 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\ 
%   Tulip & 4 & 0 & 0 & 0 & 0 & 0 & 14 & 0 & 0 & 0 & 0 & 6 & 0 & 0 & 0 & 0 & 0 & 0 & 2 & 1 & 3 \\ 
%   Vegetable & 0 & 19 & 1 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\ 
%   Winter barley & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\ 
%   Winter wheat & 0 & 0 & 23 & 26 & 0 & 3 & 0 & 20 & 8 & 10 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 \\ 
%   \hline
% \end{tabular}
% }
% \label{tab:numFOcropnBBCH}
% \end{table}

%Table \ref{tab:numFOcropnBBCH} shows a similar but different information - the number of field observations per each crop type by BBCH stage. This table is instrumental to delivering information about which crops would be possible targets for phenology tracking. For crops that have little consecutive observations over BBCH stages, we cannot carry out subsequent analysis as there is no ground-truth, which could be used as a training set. 


%\subsubsection{Close-up Pictures}
%The close-up pictures taken with the Nikon cameras represent the most high-quality piece of the data set. They represent both panoramic scenes of the whole field, similar to their street-level counterparts and close-up high-definition images of the crops in their relevant stage of development. The close-up images are tagged with each filed observation in order to know which images were taken during each observation. As of presently, the close-up pictures are not part of the study, but will be shared as part of the data set.   


% \begin{figure}
% \centering
% \hspace*{-4.9cm} 
% \begin{subfigure}{.9\textwidth}
%   \centering
%   \includegraphics[width=.9\linewidth]{figures/uapaf1Crop.png}
%   \caption{\ac{PA}/\ac{UA}/F1 for crops classes on picture level}
%   \label{fig:cMatrixCrop}
% \end{subfigure}%
% \begin{subfigure}{.9\textwidth}
%   \centering
%   \hspace*{-3.1cm} 
%   \includegraphics[width=.9\linewidth]{figures/uapaf1CropParcels.png}
%   \caption{\ac{PA}/\ac{UA}/F1 for crops classes on parcel level}
%   \label{fig:cMatrixCropParcels}
% \end{subfigure}
% \caption{Precision, Recall and \ac{F1} score for crop recognition at picture and larcel level}
% \label{}
% \end{figure}

    % \begin{figure*}
    %     \centering
    %     \begin{subfigure}[b]{0.475\textwidth}
    %         \centering
    %         \includegraphics[width=\textwidth]{figures/prc_bbchpic_py.png}
    %         \caption[]%
    %         {{\small M-PRC for 19 crop+BBCH classes on picture level}}    
    %         \label{fig:PRCgraphBBCHPIC}
    %     \end{subfigure}
    %     \hfill
    %     \begin{subfigure}[b]{0.475\textwidth}  
    %         \centering 
    %         \includegraphics[width=\textwidth]{figures/prc_bbchpar_py.png}
    %         \caption[]%
    %         {{\small M-PRC for 19 crop+BBCH classes on parcel level}}    
    %         \label{fig:PRCgraphBBCHPAR}
    %     \end{subfigure}
    %     \vskip\baselineskip
    %     \begin{subfigure}[b]{0.475\textwidth}   
    %         \centering 
    %         \includegraphics[width=\textwidth]{figures/prc_croppic_py.png}
    %         \caption[]%
    %         {{\small M-PRC for 10 crop classes on picture level}}    
    %         \label{fig:PRCgraphCROPPIC}
    %     \end{subfigure}
    %     \hfill
    %     \begin{subfigure}[b]{0.475\textwidth}   
    %         \centering 
    %         \includegraphics[width=\textwidth]{figures/prc_croppar_py.png}
    %         \caption[]%
    %         {{\small M-PRC for 10 crop classes on parcel level}}    
    %         \label{fig:PRCgraphCROPPAR}
    %     \end{subfigure}
    %     \caption[]
    %     {\small } 
    %     \label{fig:m-prc-all}
    % \end{figure*}




%\subsection{June - N sample}
%The preliminary results are concerned with taking a sample of the data-set, consisting of all the images, for which \textit{in-situ} has been collected for the month of June for 6 of the observed crops (Table \ref{table:subsetJune}, \textbf{Pictures surveyed} column). Results here were achieved while running Mobile Net module \textit{v2\_100\_224\_2}. The first obvious parameter to experiment with was the bin size of the training data-set. Tests were ran with bin sizes of 100, 300, and 500 images per crop type, while tracking labeling accuracy per individual image and per field (based on a majority vote) and processing time for both training and labelling. 

%TABLE

%Of interest was to track and try and investigate the reason for unsuccessful classifications - both for individual images and for fields. In this case the labelled test set is split into \underline{totally correctly} labelled fields, where every image of a field was correctly labelled, \underline{correctly} labelled fields, where the majority of the images were correctly labelled, \underline{incorrectly} labelled fields, where the majority of images were incorrectly labelled, and \underline{totally incorrectly} labelled fields, where all images were labelled incorrectly. Visual inspection of each image in its own context, in the context of the field it pertains to, and in context to other respectively correctly or incorrectly labelled images reveled a number of possible (connected) reasons for the relevant classification outcome:

%\begin{itemize}
    %\item crop is displayed on a relatively small part of the image
    %\item presence of soil belt around parcel
    %\item linear elements present on image (trees, hedges, etc)
    %\item presence of road elements
    %\item change in proximity to parcel throughout track
    %\item crop in early stage is too homogeneous in texture and color with surrounding vegetation
    %\item images taken for a field from the other side of the road
%\end{itemize}

%In \ref{Fig:trainingSize} we see the distribution of accuracy across the test set for three distinct training bin sizes (100, 300, 500). Irrespective of the  training set size all the runs exhibit a clear bimodal distribution of values with two distinct local maxima. We see that the majority of values are concentrated around a 0.4 probability line with the other big chunk around the 0.8 mark. Considering the fact that a 0.4 probability rate is quite low and coming from a perspective that the network is not too sure about its classification in these cases, we decide to exclude these values and set a filter of probability more than or equal to 0.65. By doing this we hope to reduce the amount of inherent error in our classification output and keep only those images, for which we feel the network is relatively sure about. In doing so, it is understandable that pictures for certain parcels might all be excluded and thus information about that parcel will be lost. This is, however, preferable to having a wrong output. On average (between test runs) the filter set on 0.65 probability rate reduces the amount of observable parcels with 2.66 \% (or 4 parcels). A trade-off exists between how high we set the threshold thus increasing the level of certainty of results, and the number of parcels that are going to be observable. 

%Furthermore, visual inspection of both correctly and incorrectly labelled images revealed a shortcoming of the random selection of input training images - inside the pool per class, it would happen that even though an image is labelled as showing a crop due to its proximity to the field, in reality there was a visual obstruction to the parcel, be it in the form of a road, a vehicle or linear elements (hedges, rows of trees). Because random selection for input while training is the preferred norm (ref), but faulty input understandably brought about faulty outcome, and because manually checking all input images to make sure they were good was not feasible (especially when scaled), we decided to introduce a class for each of the visual obstructions. As such, we imagine, if an overbearing amount of the image is taken up by one of these obstructions, the image would be labelled as showing the obstruction and not the crop. In this way we hope to prevent faulty learning and labelling and increase result robustness.  

% % latex table generated in R 3.5.2 by xtable 1.8-3 package
% % Thu Mar  7 19:53:58 2019
% \begin{table}[ht]
% \centering
% \begin{tabular}{rrrr}
%   \hline
%  & probability & meanAccChange & meanParLost \\ 
%   \hline
% 21 & 0.00 & 0.01 & -0.00 \\ 
%   22 & 0.05 & 0.01 & -0.00 \\ 
%   23 & 0.10 & 0.01 & -0.00 \\ 
%   24 & 0.15 & 0.01 & -0.00 \\ 
%   25 & 0.20 & 0.01 & -0.00 \\ 
%   26 & 0.25 & 0.01 & -0.00 \\ 
%   27 & 0.30 & 0.02 & -0.00 \\ 
%   28 & 0.35 & 0.01 & -0.00 \\ 
%   29 & 0.40 & 0.01 & 1.00 \\ 
%   30 & 0.45 & 0.04 & 2.00 \\ 
%   31 & 0.50 & 0.05 & 2.00 \\ 
%   32 & 0.55 & 0.06 & 5.00 \\ 
%   33 & 0.60 & 0.06 & 6.00 \\ 
%   34 & 0.65 & 0.05 & 10.00 \\ 
%   35 & 0.70 & 0.06 & 23.00 \\ 
%   36 & 0.75 & 0.08 & 32.00 \\ 
%   37 & 0.80 & 0.10 & 44.00 \\ 
%   38 & 0.85 & 0.09 & 60.00 \\ 
%   39 & 0.90 & 0.13 & 93.00 \\ 
%   40 & 0.95 & 0.15 & 133.00 \\ 
%   \hline
% \end{tabular}
% \end{table}

% \begin{figure}[H]
%     \centering
%     \label{Fig:trainingSize}
%     \begin{subfigure}[b]{0.3\linewidth}
%         \centering
%         \includegraphics[width=\textwidth]{./figures/Results__june_6class_n100_mobilenet_v2_100_224_2_E4000_FIG_MaxProbalitiesPerClassDistribution.png}
%         \caption{100}
%         \label{fig:FieldRevisitMap}
%     \end{subfigure}%
%     ~
%     \begin{subfigure}[b]{0.3\linewidth}
%         \centering
%         \includegraphics[width=\textwidth]{.figures/Results__june_6class_n300_mobilenet_v2_100_224_2_E4000_FIG_MaxProbalitiesPerClassDistribution.png}
%         \caption{300}
%         \label{fig:FieldRevisitTime}
%     \end{subfigure}%
%     ~ 
%         \begin{subfigure}[b]{0.3\linewidth}
%         \centering
%         \includegraphics[width=\textwidth]{.figures/Results__june_6class_n500_mobilenet_v2_100_224_2_E4000_FIG_MaxProbalitiesPerClassDistribution.png}
%         \caption{500}
%         \label{fig:FieldRevisit_january}
%     \end{subfigure}%
% \caption{Effect of the number of training sample on the distribution}
% \label{fig:FieldRevisit}
% \end{figure}


%\subsubsection{Mobilenet 0.5 224 }

